RaD-VIO: Rangefinder-aided Downward Visual-Inertial Odometry

State-of-the-art forward facing monocular visual-inertial odometry algorithms are often brittle in practice, especially whilst dealing with initialisation and motion in directions that render the state unobservable. In such cases having a reliable complementary odometry algorithm enables robust and resilient flight. Using the common local planarity assumption, we present a fast, dense, and direct frame-to-frame visual-inertial odometry algorithm for downward facing cameras that minimises a joint cost function involving a homography based photometric cost and an IMU regularisation term. Via extensive evaluation in a variety of scenarios we demonstrate superior performance than existing state-of-the-art downward facing odometry algorithms for Micro Aerial Vehicles (MAVs).

==> ieeeconf/integration.tex <==

\section{RaD-VIO and VINS-Mono Integration}
Facing the strength and weakness of both sliding window optimization based tracker (VINS-Mono) and homography based tracker (RaD-VIO), we intend to explore a integration method which take the advantage of both trackers. While higher degree of coupling might introduce larger performance gain where we provide the RaD-VIO output as initial guess for optimization within VINS-Mono (since it's never extremely diverging) and take the result returned by VINS-Mono to detect the pixels in one plane for RaD-VIO, an simple integration (\ref{fig:fig_integration}) which take advantage of the fact that RaD-VIO needs no initialization is shown here. Where we rely on RaD-VIO before VINS-D initializes, and provide a transform to correct the larger error VINS-D generates at the beginning. And it's made sure that during transition to VINS-D, the velocity estimation is continuous.

\begin{figure}[h]
	\centering
	\begin{subfigure}[b]{\linewidth}
		\includegraphics[width=0.49\linewidth]{../figure/integration_curve/curve11.png}
		\includegraphics[width=0.49\linewidth]{../figure/integration_curve/curve2.png}
		\includegraphics[width=0.49\linewidth]{../figure/integration_curve/curve12.png}
		\includegraphics[width=0.49\linewidth]{../figure/integration_curve/curve3.png}
		\includegraphics[width=0.49\linewidth]{../figure/integration_curve/curve13.png}
		\includegraphics[width=0.49\linewidth]{../figure/integration_curve/curve4.png}
	\end{subfigure}
	\caption{Comparison of velocity and position between VINS and integration mode. The dashed line highlights the switch time.}
	\label{fig:fig_integration}
\end{figure}

